Scaling Language Model Size in Cross-Device Federated Learning

Most studies in cross-device federated learning focus on small models, due to the server-client communication and on-device computation bottlenecks. In this work, we leverage various techniques for mitigating these bottlenecks to train larger language models in cross-device federated learning. With systematic applications of partial model training, quantization, efficient transfer learning, and communication-efficient optimizers, we are able to train a $21$M parameter Transformer and $20.2$M parameter Conformer that achieve the same or better perplexity as that of a similarly sized LSTM with $\sim10\times$ smaller client-to-server communication cost and $11\%$ lower perplexity than smaller LSTMs commonly studied in literature.

==> main_mar_2022.tex <==


\begin{abstract} 
% Federated learning enables training a global model on data distributed across clients.
% At each round of federated learning, the server sends the model to a subset of clients and these clients update the model using their local data and send the updated model back.
% Since clients are often edge devices, communication and computation efficiency are paramount for federated learning.
%Hence, most studies in federated learning focus on small models.
% In this work, we study the feasibility of training large language models with federated learning and evaluate various techniques to overcome communication and computation bottlenecks.
Most studies in cross-device federated learning focus on small models, due to the server-client communication and on-device computation bottlenecks. In this work, we leverage various techniques for mitigating these bottlenecks to train larger language models in cross-device federated learning. With systematic applications of partial model training, quantization, efficient transfer learning, and communication-efficient optimizers, we are able to train a $21$M parameter Transformer that achieves the same perplexity as that of a similarly sized LSTM with $\sim10\times$ smaller client-to-server communication cost and $11\%$ lower perplexity than smaller LSTMs commonly studied in literature.

% With systematic applications of partial model training, quantization, efficient transfer learning, and communication-efficient optimizers, we are able to train a $21$M parameter Transformer that achieves $11\%$ lower perplexity than a $4.7$M LSTM
% % with $146\%$ higher total communication cost of training,
% with less than half the upload communication cost per round.   
\end{abstract}

%####### 
\section{Introduction}

Federated learning is a distributed training technique, where a model is trained on data distributed across clients or edge devices without user-generated data ever leaving the device, providing an additional layer of privacy and security \citep{konevcny2016federated,konecny2016federated2, mcmahan2017communication}.
We refer readers to \cite{li2019federated, kairouz2019advances} for a detailed literature survey on federated learning.
Federated learning has been used in several applications including virtual keyboard applications \citep{hard2018federated}, keyword spotting \citep{fedkeyword2020}, and healthcare \citep{brisimi2018federated}.
%, and vehicle communication \citep{samarakoon2018federated}. 

Language models (LM) have many uses in language-based applications including virtual keyboard \citep{chen-etal-2019-federated, Zhang2021PositionInvariantTW} and automatic speech recognition %(ASR)
\citep{kannan2018externallm,variani2020hybrid,conformerlm}.
% In touch-screen keyboards, they can enhance text entry by improving next-word-prediction, decoding, and even predicting whole replies \citep{kannan2016smart}.
% In automatic speech recognition (ASR), they can improve the system by computing an external language model score during beam search inference \citep{kannan2018externallm, variani2020hybrid,conformerlm}.
Recently, there has been increased interest in training progressively larger and deeper LMs with impressive quality improvements in downstream tasks, including question answering, text classification, and text summarization \citep{devlin-etal-2019-bert,dai-etal-2019-transformer,zhilin2019xlnet,irie2019deeplmtransformer,kaplan2020scaling}.
These models tend to be variants of the Transformer \citep{vaswani2017}.
% , that relies on attention mechanisms to eliminate recurrence.
% This shift towards larger models is described by \citet{kaplan2020scaling} who note that the performance of language models generally follows scaling laws between size and cross-entropy loss.
% Previous work has also shown that for Transformers, depth is essential for better quality \citep{irie2019deeplmtransformer}.
% deeper Transformers perform significantly better than their shallower variants \citep{irie2019deeplmtransformer}. 

Federated learning is typically studied in two scenarios: \emph{cross-silo}, where the number of clients is small, and \emph{cross-device}, where the number of clients can be in the order of millions \citep{hard2018federated}.
In this work we focus on cross-device, where devices are typically edge devices such as cell phones, with limited computation and communication capabilities.
Hence, the major benchmark LMs tend to be very limited in size \citep{mcmahan2017communication,mcmahan2018learning, caldas2019leaf, reddi2020adaptive,sim21_interspeech} because memory, computation, and communication are critical bottlenecks \citep{kairouz2019advances}.
In particular, previous works that train federated LMs in production settings have used coupled input forget gate (CIFG) long short-term memory (LSTM) models with fewer than 4 million parameters \citep{hard2018federated,chen-etal-2019-federated,ramaswamy2020training}. 
% For example, \cite{hard2018federated} uses a coupled input forget gate (LSTM) long short-term memory (LSTM) model with 1.4 million parameters for next word prediction for Gboard.
% \cite{ramaswamy2020training} also uses a similar architecture for training language models with differential-private (DP) \fedavg.
% \cite{chen-etal-2019-federated} also reports training with a few LSTM LSTM architectures that are within 3.4 million parameters and subsequently converting those neural models to smaller and faster finite state transducers (FST) for virtual keyboard decoding.
These resource constraints have motivated research into various efficient algorithms for training larger models with federated learning \citep{konevcny2016federated,hamer2020fedboost}.
However, most of these techniques are still evaluated on relatively small models compared to their server-based counterparts.
In this work, we systematically evaluate multiple strategies for mitigating communication and computation costs of training larger LMs to determine if the impressive quality gains from larger models can also be achieved in cross-device federated learning. 
% to evaluate whether the impressive quality gains from larger models can also be sustained in federated learning.

While there are previous works on \emph{efficient} Transformers \citep{tay2020efficient,tay2021long}, we forgo these efficient variants as they may actually be more inefficient when sequences are short \citep{katharopoulos2020transformers,choromanski2021rethinking}.
Additionally, \citet{lin2020ensemble, liu2020federated, hilmkil2021scaling} trained large Transformer models in the cross-silo setting, where devices have more resources, whereas we focus on the resource-constrained cross-device setting. 

Recent large LMs, such as GPT-3 \cite{gpt3}, contain hundreds of billions of parameters, which is substantially bigger than the memory limits of edge devices.
Therefore in this work, we consider \emph{large} models to be at most $25$ million parameters, which is still considerably larger than existing models trained on-device. 
% TODO: We should note that efficient Transformers...
% Survey of efficient Transformers but only examine sequences of extremely long lengths \citep{tay2020efficient,tay2021long}.
% Efficient Transformer implementations that might actually have worse performance depending on if sequence length is too short \citep{child2019generating,katharopoulos2020transformers,choromanski2021rethinking}.

% On the other hand, LMs that are used for ASR are typically in the order of a hundred thousand to a few million parameters. For example, the external LM used for Listen, Attend and Spell (LAS) in \citep{kannan2018externallm} has varied sizes in the order of a few GBs. Additionally, the conformer LM used for lattice rescoring is 0.13G \citep{conformerlm}. 

% \section{Related Work}


The rest of the paper is organized as follows. In Section~\ref{sec:contrib}, we overview our contributions.
In Section~\ref{sec:data_model}, we detail the dataset and models.
We then analyze techniques to reduce the per-round cost in Section~\ref{sec:per_round_cost}, and the number of communication rounds in Section~\ref{sec:num_rounds}.
Finally in Section~\ref{sec:combination}, we combine techniques and demonstrate that large Transformers can be trained using many fewer rounds and significantly lower communication and computation cost. 

\section{Our contributions}
\label{sec:contrib}

We explore two regimes: small models typically studied in cross-device federated learning with fewer than $5$M parameters and new larger models with at most $25$M parameters. We study two architectures: CIFG-LSTM \citep{hochreiter1997}, or LSTM for simplicity, \citep{hard2018federated} and Transformer \citep{vaswani2017}. Our contributions are the following:

\begin{itemize}
    \item We are the first to investigate Transformer LMs with 25M parameters for cross-device federated learning, which we find outperform LSTMs of similar size.
    \item We demonstrate that large models substantially outperform small models on standard tasks but at much higher communication and computation costs, requiring $4\times$ the communication cost per round.
    % to reach a similar perplexity as a small LSTM. 
    % Although large models need $3$K rounds of federated training to match the perplexity of a small LSTM trained for $10$K rounds, they require $4\times$ the communication cost per round and higher memory usage.
    % \item Our experiments show that large models incur higher communication and computation costs. They transmit roughly $150$ megabytes per round and may need $10$K+ rounds to converge, which is $4\times$ the communication cost per round and $2\times$ the number of rounds compared to smaller models. Furthermore, the memory usage for clients will be much higher for the larger models.
    \item We investigate quantization and partial model training to address the per round communication and computation cost. With quantization, we achieve similar perplexity with half the download cost and one quarter of the upload cost, reducing total communication cost by $62.5\%$. Partial model training can further reduce the upload cost by $60\%$.
    \item We study transfer learning as a method of reducing the number of communication rounds and show that centralized pretraining on a suitable alternate corpus reduces the total communication rounds by $3\times$.
    \item We show that the combination of above techniques can be used to train a Large Transformer with the same perplexity as that of a similarly sized LSTM with $\sim 10\times$ the smaller client-to-server communication cost. 
\end{itemize}

% , or up to $4.7$ with small regressions

% We focus on two regimes: small models typically studied in cross-device federated learning with fewer than $5$M parameters and new larger models with at most $25$M parameters.
% We study two architectures: CIFG-LSTM \citep{hochreiter1997}, or LSTM for simplicity, \citep{hard2018federated} and Transformer \citep{vaswani2017}.
% % We note that while $25$M parameters might be still small compared to state of the art large language models, they are significantly larger compared to existing model architectures that are trained using on-device learning techniques.

% % We first ask which models perform better on standard datasets?
% We first show that large models substantially outperform small models on standard tasks, beating the perplexity of a small LSTM trained for $10$K rounds of federated training after only $3$K, and that Transformers outperform LSTMs in this regime.
% However, we also show that the large models incur higher communication and computation costs.
% They transmit roughly $150$ megabytes per round and may need $10$K+ rounds to converge, which is $4\times$ the communication cost per round and $2\times$ the number of rounds compared to smaller models.
% Furthermore, the memory usage for clients will be much higher for the larger models.
% We study existing techniques to mitigate these two issues.

% % We first show that large models substantially outperform small models on standard tasks and that Transformers outperform LSTMs in this regime.
% % While this result is encouraging and shows room for improvement for existing models, we also show that the large models incur much higher communication and computation costs.
% % In particular, we need to transmit roughly $100$ megabytes per round for around $10$K rounds, which is $4\times$ the communication cost and $3\times$ the number of rounds compared to smaller models.
% % Furthermore, the memory usage for clients will be much higher for the larger models.
% % In light of this, we study existing techniques to overcome these constraints.

% \textbf{Cost per round}:
% We investigate quantization and partial model training to reduce the per round communication and computation cost.
% Quantization allows us to achieve similar perplexity with half the download cost and one quarter of the upload cost, reducing total communication cost by a factor of $2.6$, or up to $4.7$ with small regressions.
% Partial model training can further reduce the upload cost up to $60\%$.

% \textbf{Number of communication rounds}:
% We study transfer learning as a method of reducing the number of communication rounds and show that centralized pretraining using a suitable alternate corpus reduces the total communication rounds by $3\times$. 

\section{Dataset and models}
\label{sec:data_model}

In this section, we describe the models and dataset used in the rest of the paper.
We train on the Stack Overflow federated dataset from \citet{tff}, which contains posts from the public forum grouped by username. 
Following trends in training Transformers, we use sentence-piece \citep{kudo-richardson-2018-sentencepiece} for sub-word tokenization with a vocabulary size of $4$K.
The sentence-piece model is computed based on the entire Stack Overflow training corpus in an offline process on server.
During federated learning, this fixed sentence-piece model is transmitted to each client to encode the local text data.
Doing so provides greater coverage for cross-dataset applications as well as potential downstream speech applications such as ASR \cite{li2021,sim21_interspeech}.
% Given the previous sub-words of a sentence, the goal is to predict the next sub-word.
% We measure the performance of this task in terms of test perplexity. 
We measure performance on next-subword prediction using test perplexity.
See Appendix~\ref{app:data_model} for descriptive dataset statistics. 
All experiments were implemented using JAX \citep{jax2018github} and FedJAX \citep{ro2021fedjax} federated simulation libraries.

We first did a hyperparameter search for each model and size ($\leq5$M and $\leq25$M), with FedAdam \citep{reddi2020adaptive}, or FedAvg for simplicity, 
%which combines federated averaging (FedAvg) \citep{mcmahan2017communication} with an Adam optimizer on the server \citep{kingma2015adam}, 
% using a vanilla SGD optimizer on the clients
with $200$ clients per round for $3$K rounds, resulting in four models: \emph{Small LSTM} ($4.7$M), \emph{Large LSTM} ($18.8$M), \emph{Small Transformer} ($4.1$M), and \emph{Large Transformer} ($21$M).

We then trained the chosen architectures with $800$ clients per round for $10$K rounds in Figure~\ref{fig:fedavg-baseline}.
As expected, the larger variants significantly outperform their smaller counterparts with the Large Transformer achieving the best perplexity.
However, the larger models are more expensive to train per round and although the Large Transformer achieves the best perplexity, it only surpasses the Large LSTM after $4$K rounds.
Next, we focus on techniques to reduce this cost per round and number of rounds.
For more details about the architecture search, the selected models, and their performance, see Appendix~\ref{app:data_model}. 

\begin{figure}
\centering
\includegraphics[scale=0.42]{so_fedavg.png}
% \includegraphics[scale=0.315]{so_small_fedavg.png}
% \includegraphics[scale=0.315]{so_large_fedavg.png}
\caption{Test perplexity over communication rounds for each class and size of model.}
\label{fig:fedavg-baseline}
% \vspace{-0.5cm}
\end{figure}

% As a baseline, we train each setup using  server optimizer and $800$ clients per round for $10$K rounds
% and vary the number of clients per round from $200$, $400$, and $800$ to observe speed of convergence and overall communication cost.
% For more details on learning hyperparameter selection and settings, see Appendix~\ref{app:base-search}.
% For each fixed architecture, we also sweep over various client and server learning rates while fixing the maximum number of examples per client to $1200$ or $1$ epoch and use a fixed batch size of $16$.
% We also experiment with and without applying gradient norm clipping since it may be needed for the recurrent-based LSTM \citep{pascanu2013difficulty} but not necessarily the Transformer. 
% and Table~\ref{tab:fedavg-baseline}.

% In this section, we describe and evaluate efficient methods for training large language models in the cross-device federated learning setting.
% These efficient methods address either the on-device training computation cost or communication cost (per-round download and upload of model between server and clients and total communication rounds for convergence) bottlenecks of federated learning.
% % These efficient methods focus on addressing key bottlenecks in training and deploying models via cross-device federated learning, including communication-efficiency and model latency in both training and inference.
% In particular, we examine \emph{partial model training} for on-device training computation and communication cost and \emph{quantization}, \emph{efficient transfer learning}, and \emph{communication-efficient optimization} for communication cost.
% For the most part, these techniques are orthogonal and can be combined to achieve potentially greater efficiency improvements.





% \textbf{Base architecture search}:

% We report perplexity and in-vocab-accuracy, where in-vocab-accuracy is the number of correct predictions, without UNK (out-of-vocabulary) or EOS (end-of-sentence) tokens, divided by the number of words without the EOS token.

% For LSTM and Transformer at each size range, we search over architectures and select the best performing, resulting in four models: Small LSTM ($4.7$M), Large LSTM ($18.8$M), Small Transformer ($4.1$M), and Large Transformer ($21$M).
% For details on the specific dimensions and how they were selected, see Appendix~\ref{app:base-search}.
% We determine the dimensions for each size range by conducting a sweep over hyperparameters using FedAvg with an Adam \citep{kingma2015adam} server optimizer and $200$ clients per round.
% The architectures are selected based on the final full test set perplexity after $3$K federated training rounds.
% In addition to the architecture sweep, we also do a search over client learning rates in an effort to use reasonable learning settings for the variable model sizes. 
% The details of the sweep as well as the final architectures for each class of model can be seen in Table~\ref{tab:arch-sweep}.

\section{Cost per round}
\label{sec:per_round_cost}

The larger models have $18.8$M and $21$M parameters ($150$MB and $168$MB, at $32$ bits per parameter) which need to be downloaded, trained, and uploaded at each round, a strain on both communication and computation on device. There are often strict time or transfer byte limits for each round of training, which can prohibit some devices from training these models due to slower transfer/processing speeds \citep{kairouz2019advances}.
% Naively done, this requires $32$ bits per parameter and in total $85$MB each direction (total $150$MB per round).
We show that we can significantly reduce these costs by partial model training and quantization techniques.

\textbf{Partial model training}: 
% As mentioned previously, in federated learning, training happens on device, where memory, computation, and communication are often key bottlenecks.
% Thus, reducing the cost of training is one method of reducing the computational bottleneck of training on device.
% One commonly used approach is to train only a subset of the model during training.
Training only a subset of the model can reduce the computational cost of training and has been examined in both federated \citep{caldas2019expanding,yang2021partial} and non-federated \citep{kovaleva-etal-2019-revealing} settings.
Additionally, reducing the number of trainable parameters can also decrease communication cost since only the trainable parameters need to be uploaded.
% By significantly reducing the number of trainable parameters, not only is the computational cost of training reduced but also the potential communication cost of transmitting the updated model from clients to the server, since only the trainable weights would need to be sent.

We follow the Partial Variable Training (PVT) per client per round  strategy \citep{yang2021partial} as it only freezes a subset of the original model and can be applied generally to multiple model architecture types.
% the multiplicative vectors and matrices of the original model.
% for training from scratch.
% For our partial model training experiments, we follow the Partial Variable Training (PVT) strategies proposed by \citet{yang2021partial}.
% Specifically, we use the per client per round (PCPR) configuration, where the frozen variables vary from round to round and from client to client, as this was shown to achieve the highest accuracy and work best for training from scratch.
% This corresponds to the embedding and weights of the LSTM, and for the Transformer, the weights of the MLP layer, attention matrices, layer normalization in each block, and embedding.
For more experiment details, see Appendix~\ref{app:pvt}.
We report test perplexity as a function of number of trainable variables in Figure~\ref{fig:pvt}.
Large LSTM seems to be able to handle more aggressive parameter freezing compared to Large Transformer in terms of quality regression.
However, training only $40\%$ of variables for the Large Transformer ($6.3$M) achieves better performance than the full Large LSTM ($18.8$M).

\begin{figure}
\centering
\includegraphics[scale=0.42]{so_pvt_trainable.png}
% \includegraphics[scale=0.315]{so_pvt.png}
\caption{Test perplexity as a function of number of trainable variables.}
% Bottom: Test perplexity over communication rounds for the Large language models with varying degrees of freezing. \texttt{pvt=0} indicates that the full model is trained with no freezing.
\label{fig:pvt}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{rnn_quant_download.png}
\includegraphics[scale=0.36]{large_trans_download_quant_left_leg.png}
\caption{Test perplexity over communication rounds for varying download quantization levels, with upload quantization fixed to $8$ bits. Dashed line shows the baseline without quantization.}
\label{fig:quant_download}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{rnn_upload_quant.png}
\includegraphics[scale=0.36]{trans_quant_upload.png}
\caption{Test perplexity over communication rounds for varying upload quantization levels, with download quantization fixed to $16$ bits. TernGrad is comparable to uniform with about $1.6$ bits. Dashed line shows the baseline without quantization.}
\label{fig:quant_upload}
\end{figure}

\textbf{Quantization}: 
% A straightforward method to reduce communication costs is compression of the model weights and client updates before transport.
% There are often strict time or byte limits for download and upload with each round of training, which can be mitigated by compressing data before transport, enabling more devices to participate despite slower transfer/processing speeds.
% , or time limits under which the device must download the model weights, complete a round of training, and upload gradients (TODO does this need to be motivated?).
% Compressing the data before transport can address these concerns and also allow less powerful devices to participate in training despite slower transfer or processing speeds.
To reduce communication costs, various quantization strategies can decrease the number of bits required to represent model parameters \citep{bernstein2018signsgd,pmlr-v108-reisizadeh20a,gandikota2021vqsgd,vargaftik2021drive}. We examine stochastic k-level uniform quantization \citep{alistarh2017qsgd, suresh2017distributed} as it can be applied to model parameters on download (server-to-client) and model updates on upload (client-to-server) communication with adjustable levels of compression, and compare with TernGrad, an upload technique \citep{wen2017terngrad}. 
% Removed citation: mayekar2021wyner

% Quantization is a technique commonly used to compress neural networks by reducing the number of bits used to represent the model parameters, which can cut the model size drastically with minimal effects on model accuracy (TODO insert refs).
% Quantization can also be applied to the client updates \citep{pmlr-v108-reisizadeh20a}, which are smaller in size than the model parameters but represent the tightest communication bottleneck (for example, \cite{mobile-speeds-05-2021} reports that mobile upload speeds worldwide are over 4x slower than download speeds as of May 2021).
% While our experiments for this work are done in simulation and therefore communication cost is not a priority, understanding how this method affects larger LMs will be key in translating this research into practical applications on real edge devices.

% We experiment with stochastic $$K-level uniform quantization as discussed in \cite{suresh2017distributed} for both download (server to client) and upload (client to server). For upload quantization, which is the tightest bottleneck in practice, we also explore zero-centering before compression, as well as L-infinity clipping. Additionally, we try an alternative to uniform quantization, TernGrad, a method that quantizes values into 3 levels \citep{wen2017terngrad}.

% In stochastic $$K-level uniform quantization \cite{suresh2017distributed}, values in each layer are converted into one of $$K evenly distributed values between the layer min and max, stochastically assigned to the closest target value either above or below the real value.
% The lower the $$K value, the more the data is being compressed, as the number of bits used to store the value equals $log(k)$.
% For download quantization, we explore $$K values corresponding to between 8 and 28 bits.
% For upload quantization which as we mentioned can be more of a bottleneck, we explore $$K values corresponding to between 1 and 28 bits.

% We perform additional experiments to explore upload quantization in more detail. We try quantizing after applying L-infinity clipping to 2.5 standard deviations and/or zero-centering the values. We also try TernGrad \cite{wen2017terngrad}, where each value is converted into either 0 or the $+/-$ greatest magnitude value of the layer ($max(abs(v))$. We compare this to uniform quantization into 3 levels (1.585 bits). For simplicity, we applied TernGrad to all layers instead of leaving the last layer uncompressed as \citep{wen2017terngrad} did with their larger scale experiments (TODO although we should try in future work...?). We experiment with and without the same L-infinity clipping here as well.

% For stochastic k-level uniform quantization, we try download bits from $8$ to $28$ and bits from $1$ to $28$ for upload, the larger bottleneck in edge devices \citep{mobile-speeds-05-2021}.
% On upload, we also try applying L-infinity clipping and zero-centering as well as TernGrad, which uses $\log_2(3)$ bits per parameter.


% We found that smaller models see less regression in perplexity compared to their baseline than larger models, which we were expecting, and as quantization is mainly a technique to allow training larger models we focus this analysis on the $\si$M20M parameter models. We did notice something unexpected -- the LSTM model seemed more "quantizable" during download than the Transformer models, in that applying more aggressive quantization (into a smaller number of bits) resulted in less regression from the baseline compared to the Transformer. Figure~\ref{fig:quant_download} shows the gap between each pair of curves is larger for the Transformer than the LSTM. Using at least 16 bits for download quantization performs very close to the baseline.

We focus analysis on larger models which are more affected by quantization. The LSTM appears more "quantizable" during download than the Transformer, with less regression in Figure~\ref{fig:quant_download}. 
The perplexity of the Transformer with $16$ download bits matches that of the baseline Transformer and with $12$ bits its perplexity is close to that of the LSTM.
%$16$ download bits meets the baseline, with $12$ bits close behind in the LSTM.
For both the models, $8$ bit upload matches the corresponding baselines, or even $6$ bits for the LSTM in Figure~\ref{fig:quant_upload}. TernGrad, requiring $\log_2(3)$ bits, outperforms the $4$ bit in the Transformer but not for the LSTM in Figure~\ref{fig:quant_comm_costs}.
% TernGrad, requiring $\log_2(3)$ bits, performs much better than the uniform $2$ bit thanks to its $\ell_\infty$ clipping, which we found critical when using lower bits.
More details are in Appendix~\ref{app:quant}.
%, as long as L infinity clipping is applied. Clipping appears to have a much larger impact in the Transformer than in the LSTM, where Terngrad performs worse than 4-bit. 

% Zero-centering did not seem to affect upload behavior much for either model, marginally improving the LSTM and marginally degrading the Transformer.


\begin{figure}[t]
\centering
\includegraphics[scale=0.42]{quant_comm_costs_large_focus.png}
\caption{Test set perplexity versus total communication cost (download $+$ upload) in a single round of training, for each quantization algorithm. Uniform settings include points for varying quantization bits.}
\label{fig:quant_comm_costs}
\end{figure}

\section{Number of communication rounds}
\label{sec:num_rounds}
\textbf{Transfer learning}: 
% Another category of efficient methods for reducing the  cost of training larger models on device for federated learning is efficient transfer learning.
Transfer learning leverages pretrained models to improve model quality \citep{pmlr-v97-houlsby19a}.
By pretraining, the number of communication rounds required for model convergence can be significantly reduced \citep{stremmel2020pretrain}.
% Following pretraining, we fine-tune the entire model, but it has been shown that a smaller subset of the model can be fine-tuned without a large drop in quality \citep{lee2019elsa}.


We use two datasets for pretraining: a large corpus of digitized books \citep{Zhang2021PositionInvariantTW} and the One Billion Word Benchmark (LM1B) \citep{Chelba2014OneBW}.
After pretraining using synchronous SGD for $30$M steps, we finetune on Stack Overflow using FedAvg.
For additional details, see Appendix~\ref{app:transfer}.
We report results for each of the pretraining datasets and random initialization in Figure~\ref{fig:pretraining}.
Books consistently outperforms LM1B for both the LSTM and Transformer.
Pretraining greatly benefits the Large Transformer compared to the Large LSTM, reducing the number of rounds needed to reach the final $10$K without pretraining by $4$K rounds.
Furthermore, at round $2$K, the Large Transformer already outperforms the Large LSTM, making the number of rounds needed for training similar to that of smaller models used in mobile keyboard prediction \citep{hard2018federated}. 
% As we train for more rounds, the benefits of pretraining diminishes.
% As shown in Figure~\ref{fig:pretraining}, at round $10$K the Books pretrained Large Transformer model is only slightly better than its randomly initialized counter part. Training on more labeled data has been shown to diminish the value of pretraining in computer vision tasks as well \citep{rethinkingpretraining2020}.

% Specifically, we vary fine-tuning the last $$K layers of the model.
% Thus, using efficient transfer learning strategies, not only can the overall communication cost be reduced but also the computational cost of training on device.

\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{large_lstm_pretrain.png}
\includegraphics[scale=0.36]{large_trans_pretrain.png}
\caption{Test perplexity over communication comparing pretraining corpora. Dashed line is the final perplexity reached by the randomly initialized model.}
\label{fig:pretraining}
\end{figure}



% \begin{figure}
% \centering
% \caption{Test set perplexity over communication rounds for each class of language model.}
% \label{fig:transfer}
% \end{figure}

%TODO: Explain experiments setup.

% Results are in Figure~\ref{fig:transfer} and Table~\ref{tab:transfer}.

\textbf{Different optimizers}: 
Since the introduction of FedAvg, several variations continue to be developed \citep{li2018federated,hamer2020fedboost,reddi2020adaptive}.
% Even if the per-round cost is low, there can still be a communication bottleneck if many rounds are required for convergence. 
Specifically, we examine MimeLite \citep{karimireddy2020mime} and FedProx \citep{li2018federated} as they have been shown to reduce the total amount of rounds required for provable convergence.
% By cutting the amount of required federated training rounds, the total communication cost of federated training can be drastically reduced, especially when communicating larger model sizes.
% Note that we only use MimeLite rather than the base Mime algorithm due to lower communication cost since MimeLite only requires a single round of communication between server and client per federated training round.
However, in Figure~\ref{fig:comm-opt}, FedProx and MimeLite do not improve convergence speed over FedAvg.
More details can be found in Appendix~\ref{app:comm-opt}.

\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{so_lstm_opt.png}
\includegraphics[scale=0.36]{so_trans_opt.png}
% \includegraphics[scale=0.315]{so_commopt.png}
% \includegraphics[scale=0.315]{so_small_commopt.png}
% \includegraphics[scale=0.315]{so_large_commopt.png}
\caption{Test perplexity over communication rounds for each model and algorithm.}
\label{fig:comm-opt}
\end{figure}

\section{Combination of techniques} 
\label{sec:combination}
% Given the positive results observed in our experiments with partial model training, quantization, and efficient transfer learning, and their orthogonal nature,
We experiment with combining partial model training, quantization, and transfer learning to train \emph{efficient} larger models.
For these experiments, we train on just $40\%$ of trainable parameters with PVT
% apply $16$ bit uniform quantization on the download
% apply $8$ bit uniform quantization on the upload,
and warm start after pretraining on the Books corpus.
Combining download quantization with these techniques did not perform as well, so we only apply $8$ bit uniform quantization on upload, which is the tightest communication bottleneck (\citet{mobile-speeds-05-2021} reports that mobile upload speeds worldwide are over $4\times$ slower than download as of May 2021).
For the full experiment details, refer to Appendix~\ref{app:combo}.
% We also note that by combining PVT and quantization, upload cost can be further reduced as only the updates need be uploaded.
We report the test perplexity in terms of total upload communication cost in Figure~\ref{fig:combo-upload}.
% as it has been shown that upload is the tightest communication bottleneck (\citet{mobile-speeds-05-2021} reports that mobile upload speeds worldwide are over 4x slower than download speeds as of May 2021).
% Try to make this clearer that we're comparing at a given X-value not the final value
Restricting for small upload costs ($<200$GB), the efficient models outperform all others with the efficient Large Transformer yielding the best perplexity.
Furthermore, the efficient Large Transformer also achieves the same  perplexity as the Large LSTM with no efficient techniques. 



\begin{figure}[t]
\centering
\includegraphics[scale=0.42]{so_combo.png}
\caption{Test perplexity over total uploaded gigabytes per client for each class of model.}
\label{fig:combo-upload}
\end{figure}

\section{Conclusion}

We systematically studied several techniques for addressing the communication and computation bottlenecks of federated learning.
We further demonstrated that these techniques, individually or in combination, can scale to larger models in cross-device federated learning.
% , while achieving better quality than existing smaller models.
% In particular, the Large Transformer trained with the combination of efficient techniques proved most promising.
Extending this study to other architectures and efficient strategies remains an interesting open question.
